Polynomial Identity Testing via Evaluation of Rational Functions

$ \newcommand{\ie}{i.\,e.} $We introduce a hitting set generator for Polynomial Identity Testing based on evaluations of low-degree univariate rational functions at abscissas associated with the variables. We establish an equivalence up to rescaling with a generator introduced by Shpilka and Volkovich, which has a similar structure but uses multivariate polynomials. We initiate a systematic analytic study of the power of hitting set generators by characterizing their vanishing ideals, \ie, the sets of polynomials that they fail to hit. We provide two such characterizations for our generator. First, we develop a small collection of polynomials that jointly produce the vanishing ideal. As corollaries, we obtain tight bounds on the minimum degree, sparseness, and partition class size of set-multilinearity in the vanishing ideal. Second, inspired by a connection to alternating algebra, we develop a structured deterministic membership test for the multilinear part of the vanishing ideal. We present a derivation based on alternating algebra along with the required background, as well as one in terms of zero substitutions and partial derivatives, avoiding the need for alternating algebra. As evidence of the utility of our analytic approach, we rederive known derandomization results based on the generator by Shpilka and Volkovich and present a new application in derandomization / lower bounds for read-once oblivious algebraic branching programs.

==> tocspecial.tex <==
%% tocspecial.tex 2020-09-01  Version 0.22  ToC style file
%------------------------------------------------------------------
% Filename: tocspecial.cls
% 
% This documentclass is intended for typesetting articles for the
% 
% Theory of Computing.
% 
% See http://theoryofcomputing.org for further details.
%
% Version 0.1 Initial combination of banners from previous style files.
% Version 0.2 Addition of CCC banners. Clean up.
% Version 0.21 Addition of more CCC banners, up to 2023
% Version 0.22 Rename \boolean --> \aboolean to avoid clash with ifthen.
% ------------------------------------------------------------------
%
%% Special issue banners:

%% explanation: BC = 2012 BD = 2013 ... CA = 2020 CB = 2021 ...

\newcommand{\motwani}{Special issue in honor of Rajeev Motwani}
\newcommand{\aboolean}{Special issue: Analysis of Boolean Functions}
\newcommand{\approxrandomBC}{Special issue: APPROX-RANDOM 2012}
\newcommand{\approxrandomBD}{Special issue: APPROX-RANDOM 2013}
\newcommand{\approxrandomBE}{Special issue: APPROX-RANDOM 2014}
\newcommand{\approxrandomBF}{Special issue: APPROX-RANDOM 2015}
\newcommand{\approxrandomBG}{Special issue: APPROX-RANDOM 2016}
\newcommand{\randomBI}{Special issue: RANDOM 2018}
\newcommand{\approxrandomBJ}{Special issue: APPROX-RANDOM 2019}
\newcommand{\approxrandomCA}{Special issue: APPROX-RANDOM 2020}
\newcommand{\approxrandomCB}{Special issue: APPROX-RANDOM 2021}
\newcommand{\approxrandomCC}{Special issue: APPROX-RANDOM 2022}
\newcommand{\cccBF}{Special issue: CCC 2015}
\newcommand{\cccBG}{Special issue: CCC 2016}
\newcommand{\cccBH}{Special issue: CCC 2017}
\newcommand{\cccBI}{Special issue: CCC 2018}
\newcommand{\cccBJ}{Special issue: CCC 2019}
\newcommand{\cccCA}{Special issue: CCC 2020}
\newcommand{\cccCB}{Special issue: CCC 2021}
\newcommand{\cccCC}{Special issue: CCC 2022}
\newcommand{\cccCD}{Special issue: CCC 2023}

